Temporal Knowledge Distillation for On-device Audio Classification

Improving the performance of on-device audio classification models remains a challenge given the computational limits of the mobile environment. Many studies leverage knowledge distillation to boost predictive performance by transferring the knowledge from large models to on-device models. However, most lack a mechanism to distill the essence of the temporal information, which is crucial to audio classification tasks, or similar architecture is often required. In this paper, we propose a new knowledge distillation method designed to incorporate the temporal knowledge embedded in attention weights of large transformer-based models into on-device models. Our distillation method is applicable to various types of architectures, including the non-attention-based architectures such as CNNs or RNNs, while retaining the original network architecture during inference. Through extensive experiments on both an audio event detection dataset and a noisy keyword spotting dataset, we show that our proposed method improves the predictive performance across diverse on-device architectures.

==> Sections/A_1_Common_Rebuttal.tex <==
We sincerely thank all the reviewers for their constructive feedback.
We are especially pleased that Reviewers \textit{\textbf{1610}} and \textit{\textbf{2EED}} thought our proposed method is moderately original with technical correctness and experimental results are convincing.
We are also pleased that Reviewer \textit{\textbf{00D0}} thought the descriptions and the illustrations for our method are exemplary, and Reviewer \textit{\textbf{1610}} says that the overall presentation is clear enough.
Moreover, Reviewers say that our references are adequate (\textit{\textbf{1610}}) and excellent (\textit{\textbf{2EED}}).
We will do our best to respond to the issues raised by the reviewers in this author response period.


==> Sections/A_2_Grammar_Mistakes.tex <==
\setcounter{section}{0}
\section{Minor fixes}
We thank the reviewers for pointing out the grammar issues to make our paper more clear.
We list the fixed issues including the reviewer's suggestions as follows:
\vspace*{1em}

\noindent \textbf{[Abstract]} However, most lack \textcolor{red}{a mechanism to distill} the essence of the temporal information\textcolor{red}{,} which is crucial to audio classification tasks, or similar architecture is often required.

\noindent \textbf{[Abstract]} In this paper, we propose a new knowledge distillation method designed to incorporate the temporal knowledge embedded in attention weights of large \textcolor{red}{transformer-based} models \textcolor{red}{into} \sout{to} on-device models.

\noindent \textbf{[Abstract]} Our distillation method is applicable to various types of architectures, including \sout{the} non-attention-based architectures such as CNNs or RNNs, \textcolor{red}{while retaining the original network architecture} \sout{without any architectural change} during inference.

\noindent \textbf{[Introduction]} On-device models have achieved comparable performance to \textcolor{red}{much larger} \sout{large} models on several tasks such as keyword spotting (KWS).

\noindent \textbf{[Introduction]} \textcolor{red}{Improving the performance of on-device models is challenging} \sout{It is challenging to improve the per- formance of on-device models} due to the restricted memory and computing resources in the mobile environment.

\noindent \textbf{[Introduction]} In this paper, we introduce a simple yet effective method that can distill the temporal knowledge from attention weights of large \textcolor{red}{transformer} models to on-device models of various architectures.

\noindent \textbf{[Introduction]} The noisy KWS dataset is constructed by injecting the existing KWS dataset samples (Google Speech Commands v2) into different \textcolor{red}{speech-like noise} \sout{noisy} audios, making the temporal information more important for classifying each \textcolor{red}{specific target} keyword.

\noindent \textbf{[Introduction]} Experimental results demonstrate that applying our method improves the predictive performance of various on-device models without any architectural changes during inference \textcolor{red}{by distilling temporal information during training}.

\noindent \textbf{[Teacher: Large Transformer-based Model]} We employ the XLSR-wav2vec 2.0 as our teacher model $\mathcal{F}_T$, which is \sout{a} large-scale transformer-based ASR model with \sout{a} state-of-the-art performance on multilingual ASR.

\noindent \textbf{[Student: Lightweight On-device Models]} The \textcolor{red}{extracted student} attention weights act as recipients \textcolor{red}{for transferring} \sout{of the transferred} high-level knowledge \textcolor{red}{from} \sout{of} the teacher model $\mathcal{F}_T$.

\noindent \textbf{[Student: Lightweight On-device Models]} There are many strategies for designing the query $\mathbf{q}$, e.g., random initialization or projection of the medium context representation, where we chose the latter\sout{ one}.

% \noindent \textbf{[Student: Lightweight On-device Models]} While this approach is not universally applicable for arbitrary architectures, we emphasize that the only architectural requirement for the student model to satisfy is to output \sout{an} intermediate features which preserve the temporal information.

\noindent \textbf{[Temporal Knowledge Distillation]} The attention rollout technique is applied to the self-attention maps \textcolor{red}{to result} \sout{and results} in a single unified attention map $\mathbf{A}'_T \in \mathbb{R}^{n\times n}$.

% \noindent \textbf{[Temporal Knowledge Distillation]} Therefore, we employ a simple linear interpolation method to match the dimension of $\mathbf{a}'_1$ with $\mathbf{a}_S$ while preserving the temporal knowledge.

\noindent \textbf{[Temporal Knowledge Distillation]} where the \sout{$\mathcal{L}_{cls}$} \textcolor{red}{$\mathcal{L}_{CLS}$} is a cross-entropy-based classification loss of the student model.

\noindent \textbf{[Temporal Knowledge Distillation]} Therefore, we employ a simple linear interpolation method \textcolor{red}{to resize the attention weights} to match the dimension of $\mathbf{a}'_1$ with $\mathbf{a}_S$ while preserving the temporal knowledge.

\noindent \textbf{[Temporal Knowledge Distillation]} After applying \sout{the} linear interpolation on the attention weights $\mathbf{a}'_1$, we obtain the final attention weights $\mathbf{a}*T$ of the teacher model $\mathcal{F}*{T}$.

\noindent \textbf{[Experimental Setup]} We generate the synthetic audios by injecting the one-second speech command audios \textcolor{red}{into} \sout{to} the background speech noise obtained from the \textit{``Hubbub", ``speech noise", ``speech babble"} classes of the \textit{AudioSet} dataset.

\noindent \textbf{[Experimental Setup]} The noisy datasets are split using the same \textcolor{red}{training and validation splits as} \sout{training splits with} the Speech Commands v2 dataset.

\noindent \textbf{[Experimental Setup]} The teacher model (XLSR-wav2vec 2.0) is pretrained on \textcolor{red}{a} multilingual speech dataset.

\noindent \textbf{[Experimental Setup]} We leverage \sout{an} existing code for our experiments.

\noindent \textbf{[Evaluation Results]} In Figure 2, we visualize attentions extracted from \textcolor{red}{the} teacher model and all \textcolor{red}{the} student models applied on 8 second \textcolor{red}{audio} sample from Noisy Speech Commands v2.

\noindent \textbf{[Conclusion]} In this paper, we \textcolor{red}{propose} \sout{proposed} a novel attention distillation method that transfers the temporal knowledge from large teacher models to on-device student audio classification models.

\noindent \textbf{[Conclusion]} Through extensive experiments on both an audio event detection dataset and a noisy keyword spotting dataset, we show that our proposed method improves the predictive performance\sout{. Experimental results indicate our method improves the predictive performance} of on-device models by successfully learning the attention weights from the large teacher model.


==> Sections/A_Rebuttal.tex <==
\newpage
\section*{Author Response to Reviewer \textit{1610}}
\input{Sections/A_1_Common_Rebuttal}

\input{Sections/A_2_Grammar_Mistakes}


\clearpage
\newpage
\section*{Author Response to Reviewer \textit{00D0}}
\input{Sections/A_1_Common_Rebuttal}

\vspace*{1em}
\noindent
\textbf{Recap for Our Contributions:}
Introducing an effective knowledge distillation method that transfers the temporal knowledge from attention weights of transformer-based large models to on-device models with various architectures.

\setcounter{section}{0}
\section{Responses}
\textbf{[Q] The architectural specs include ACOUSTICS in the model and SPEECH data in the training data only.}
\newline
[A] We want to emphasize that our proposed method is not limited to speech data, applicable to any audio data.
To support this claim, we show the experimental results both on the audio event detection (AED) dataset and the keyword spotting (KWS) dataset.

\vspace*{1em}
\noindent
\textbf{[Q] The authors correctly use unconventional vocabulary such as teacher and student instead of training and inference, eventually to highlight this particular feature.}
\newline
[A] We strongly believe that the term \textit{teacher and student} models are widely used in knowledge distillation (KD) literature, where the concept of teacher and student in KD is essential to our proposed method, i.e., we respectively disagree that those terms are unconventional.
In KD methodologies, both teacher and the student models are trained, and the trained teacher model transfers its knowledge to the student model when the student model is training.
Therefore, contrary to what the reviewer \textit{00D0} points out, one must strictly separate the concept of the teacher and student models from the concept of training and inference stages.


\vspace*{1em}
\noindent
\textbf{[Q] The extensive testing does not clear my doubts that the comparative study is flawed by opinionated training data.}
\newline
[A] To show the effectiveness of our proposed method, we conduct experiments on both the noise-injected dataset (\textit{noisy speech commands v2}) and the standard AED benchmark dataset (\textit{FSD50K}).
To demonstrate the importance of temporal information, we selected tasks that require analyzing long audios where both KWS and AED are challenging real-world problems for on-device models. 
Also, the commonly used on-device KWS dataset (\textit{Speech Commands v2}) only contains clean 1 second audio recordings without background noises.
We found the task to be too simple so that the on-device models are on par with their larger counterparts, as we mentioned in the manuscript.
Thus, we design the \textit{noisy speech commands v2} dataset by inserting the KWS audio samples into longer speech noise clips.
We can directly control the difficulty for on-device models to correctly classify the keywords present in the audio by changing the length of the noise audio.
Evaluation results on the noisy dataset demonstrate that our proposed method is robust to harsher but realistic conditions when speech noise is present in keyword spotting.




\vspace*{1em}
\noindent
\textbf{[Q] Also the inventors may would have to face the disclosure of their discrete linear interpolation method.}
\newline
[A] The disclosure of the interpolation method is not a concern for the authors as we utilized a commonly used method, readily available in common python libraries such as \texttt{numpy}’s \texttt{interp} function.
We will add this information in the camera-ready version to reduce confusion.


\vspace*{1em}
\noindent
\textbf{[Q] Does not cite relevant work.}
\newline
[A] We agree with other reviewers (\textit{1610} and \textit{2EED}) that this manuscript covers an adequate amount of relevant works.
Nevertheless, we will be happy to review the related papers if recommended and add them to the camera-ready version.

\clearpage
\newpage
\section*{Author Response to Reviewer \textit{2EED}}
\input{Sections/A_1_Common_Rebuttal}
\input{Sections/A_2_Grammar_Mistakes}

